Decomposition of Map Graphs with Applications

Bidimensionality is the most common technique to design subexponential-time parameterized algorithms on special classes of graphs, particularly planar graphs. The core engine behind it is a combinatorial lemma of Robertson, Seymour and Thomas that states that every planar graph either has a $\sqrt{k}\times \sqrt{k}$-grid as a minor, or its treewidth is $O(\sqrt{k})$. However, bidimensionality theory cannot be extended directly to several well-known classes of geometric graphs. Nevertheless, a relaxation of this lemma has been proven useful for unit disk graphs. Inspired by this, we prove a new decomposition lemma for map graphs. Informally, our lemma states the following. For any map graph $G$, there exists a collection $(U_1,\ldots,U_t)$ of cliques of $G$ with the following property: $G$ either contains a $\sqrt{k}\times \sqrt{k}$-grid as a minor, or it admits a tree decomposition where every bag is the union of $O(\sqrt{k})$ of the cliques in the above collection. The new lemma appears to be a handy tool in the design of subexponential parameterized algorithms on map graphs. We demonstrate its usability by designing algorithms on map graphs with running time $2^{O({\sqrt{k}\log{k}})} \cdot n^{O(1)}$ for the Connected Planar $\cal F$-Deletion problem (that encompasses problems such as Feedback Vertex Set and Vertex Cover). Obtaining subexponential algorithms for Longest Cycle/Path and Cycle Packing is more challenging. We have to construct tree decompositions with more powerful properties and to prove sublinear bounds on the number of ways an optimum solution could "cross" bags in these decompositions. For Longest Cycle/Path, these are the first subexponential-time parameterized algorithms on map graphs. For Feedback Vertex Set and Cycle Packing, we improve upon known $2^{O({k^{0.75}\log{k}})} \cdot n^{O(1)}$-time algorithms on map graphs.

==> longcycle.tex <==
%!TEX root = main_map.tex

\section{Longest Cycle}\label{sec:longCyc}

In this section, we show that \probKCycle admits a subexponential-time parameterized algorithm. More precisely, we prove the following.

\begin{theorem}\label{thm:longestCyc}
\probKCycle on map graphs can be solved in time $2^{\OO(\sqrt{k}\log k)}\cdot n^{\OO(1)}$.
\end{theorem}

We start by stating a direct implication of Lemma~\ref{lem:exactKCycle}.

\begin{corollary}\label{cor:nearKCycle}
Given a graph $G$, representation $f$ and $k\in\mathbb{N}$, it can be determined in time $2^{\OO(\sqrt{k}\log k)}\cdot n^{\OO(1)}$ whether $G$ contain a cycle whose number of vertices is between $k$ and $2k$.
\end{corollary}

\begin{proof}
Run the algorithm given by Lemma~\ref{lem:exactKCycle} with $k=\ell,\ell+1,\ldots,2\ell$, and return \Yes{} if and only if at least one of the executions returns \Yes. Correctness and running time follow directly from Lemma~\ref{lem:exactKCycle}.
\end{proof}

%Next, we examine the operation that contracts an edge. To this end, we need the following. 
%
%
%\begin{definition}\label{def:contractiblePair}
%A pair $(u,v)$ of distinct vertices $u,v\in V(G)$ is {\em contractible} if $f(u)=f(v)$.
%\end{definition}
%
%Note that if $(u,v)$ is a contractible pair, then by Condition \ref{condition:GridClique1} in Definition \ref{def:GridClique}, it holds that $\{u,v\}\in E(G)$. Now, given a contractible pair $(u,v)$, denote $e=\{u,v\}$, and define the function $f_{/e}: V(G/e)\rightarrow[t]\times[t']$ as follows. For all $w\in V(G)\setminus\{v,u\}$, define $f_{/e}(w)=f(w)$. Moreover, define $f_{/e}(x_{\{u,v\}})=f(u)$. By Definitions \ref{def:GridClique} and \ref{def:cellGraph}, we immediately have the following.
%
%\begin{observation}\label{obs:funcFe}
%The function $f_{/e}$ is a representation of $G/e$. Furthermore, $G$ and $G/e$ have the same cell graph.
%\end{observation}
%
%In particular, we deduce that $(G/e,f_{/e},k)$ is an instance of \probKCycle on \gcgraphs. Next, we note that the operation that contracts an edge preserves the answer \No---the correctness of this claim follows from the fact that $G/e$ is a minor of $G$.
%
%\begin{observation}\label{obs:longCycPreserveNo}
%Let $(G,f,k)$ be an instance of \probKCycle on \gcgraphs. Then, $(G/e,f_{/e},k)$ is an instance of \probKCycle on \gcgraphs such that if $(G,f,k)$ is a \No-instance, then $(G/e,f_{/e},k)$ is a \No-instance.
%\end{observation}
%
%Now, we also verify that in case there exists a cycle on at least $2k$ vertices, the operation that contracts an edge also preserves the answer \Yes.
%
%\begin{lemma}\label{lem:longCycPreserveYes}
%Let $(G,f,k)$ be an instance of \probKCycle on \gcgraphs{} such that $G$ contains a cycle $C$ on at least $2k$ vertices. Then, $(G/e,f_{/e},k)$ is a \Yes-instance.
%\end{lemma}
%
%\begin{proof}
%Denote $e=\{u,v\}$. In case $V(C)\cap\{u,v\}=\emptyset$, then $C$ is also a cycle in $G/e$, and in case $|V(C)\cap\{u,v\}|=1$, then by replacing the vertex in $V(C)\cap\{u,v\}$ by $x_{\{u,v\}}$ in $C$, we obtain a cycle of the same length as $C$ in $G/e$. In both of these cases, the proof is complete, and thus we next suppose that $\{u,v\}\subseteq V(C)$.
%
%Let us denote $C=v_1-v_2-v_3-\cdots-v_\ell-v_1$, where $v_1=u$ and $v_i=v$ for some $i\in[\ell]\setminus\{1\}$. Note that $\ell\geq 2k$. Without loss of generality, assume that $i-2\geq \ell-i$ (else we replace each $v_j$, except for $v_1$, by $v_{\ell-j}$, and obtain a cycle where this property holds). Now, note that $C'=x_{\{u,v\}}-v_2-\cdots-v_{i-1}-x_{\{u,v\}}$ is a cycle in $G/e$. Moreover, since $i-2\geq \ell-i$, it holds that $|V(C')|=i-1\geq\frac{\ell}{2}\geq k$. Thus, $(G/e,f_{/e},k)$ is a \Yes-instance.
%\end{proof}
%
%Before we present our algorithm, we need two additional propositions, handling the extreme cases where we either discover that our input graph contains a large grid or, after a series of operations that contracted edges in $G$, we ended up with a graph isomorhpic to the cell graph of $G$. For the first case, we need the following result (see also \cite{Demaine:2008mi,cygan2015parameterized}).
%
%\begin{observation}\label{obs:longCycLargeGrid}
%Let $(G,k)$ be an instance of \probKCycle{} on general graphs. If $G$ contains a $\sqrt{k}\times \sqrt{k}$ grid as a minor, then $(G,k)$ is a \Yes-instance.
%\end{observation}
%
%For the second case, we need the following result (see also \cite{cygan2015parameterized}).
%
%\begin{proposition}[\cite{BodlaenderCK12}]\label{prop:DPLongCyc}
%\probKCycle on graphs of treewidth $\mathrm{\it tw}$ can be solved in time $2^{\OO(\mathrm{\it tw})}\cdot n^{\OO(1)}$.
%\end{proposition}
%
%From Proposition \ref{prop:DPLongCyc} and the fact that $\cell(G)$ is a minor of $G$, we have the following.
%
%\begin{observation}\label{obs:longCycEndCell}
%Let $(G,f,k)$ be an instance of \probKCycle on \gcgraphs{}. Then, it can be determined in time $2^{\OO(\tw(\cell(G)))}\cdot n^{\OO(1)}$ whether $\cell(G)$ contains a cycle on at least $k$ vertices, in which case $(G,f,k)$ is a \Yes-instance.
%\end{observation}
%
%We are now ready to present our algorithm. The proof of correctness and analysis of running times are integrated in the description of the algorithm.
%
%\subparagraph*{Proof of Theorem \ref{thm:longestCyc}.}
%Let $(G,O,k)$ be an instance of \probKCycle on unit disk/square graphs. By using Corollary~\ref{cor:firstPhaseToGrid}, we first obtain an equivalent instance $(G,f,k)$ of \probKCycle on \gcgraphs{} (both instances refer to the same graph $G$ and parameter $k$). Next, by using Lemma~\ref{lem:mainCell} with the parameter $\ell=100\cdot599^3\cdot\sqrt{k}$, we either correctly conclude that $G$ contains a $\sqrt{k}\times\sqrt{k}$ grid as a minor, or compute a tree decomposition of $\cell(G)$ of width at most $500\cdot599^3\cdot\sqrt{k}=\OO(\sqrt{k})$. In the first case, by Observation \ref{obs:longCycLargeGrid}, we are done. In the latter case, by using Observation~\ref{obs:longCycEndCell}, we determine in time $2^{\OO(\sqrt{k})}\cdot n^{\OO(1)}$ whether $\cell(G)$ contains a cycle on at least $k$ vertices, where if the answer is positive, then we are done. Thus, we next suppose that $\cell(G)$ does not contain a cycle on at least $k$ vertices.
%
%Now, as long as there exists a contractible pair $(u,v)$, we perform the following operation. First, by using Corollary~\ref{cor:nearKCycle}, we determine in time $2^{\OO(\sqrt{k}\log k)}\cdot n^{\OO(1)}$ whether $G$ contain a cycle whose number of vertices is between $k$ and $2k$. If the answer is positive, then we are done (our final answer is \Yes). If the answer is negative, then we contract the edge $\{u,v\}$. By Lemma \ref{lem:longCycPreserveYes}, we obtain an instance that is equivalent to the previous one. Note that the loop described in this paragraph can have at most $\OO(n^2)$ iterations, and therefore its total running time is bounded by $2^{\OO(\sqrt{k}\log k)}\cdot n^{\OO(1)}$.
%
%Once there does not exist a contractible pair $(u,v)$, as we have only modified the graph by contracting edges, on at a time, between contractible pairs, we are left with a graph that is isomorphic to the cell graph of our original input graph. We have already correctly concluded that this graph does not contain a cycle on at least $k$ vertices. Thus, at this point, we correctly answer \No.\qed

